Hey AI, Generate Me a Hardware Code! Agentic AI-based Hardware Design & Verification

Modern Integrated Circuits (ICs) are becoming increasingly complex, and so is their development process. Hardware design verification entails a methodical and disciplined approach to the planning, development, execution, and sign-off of functionally correct hardware designs. This tedious process requires significant effort and time to ensure a bug-free tape-out. The field of Natural Language Processing has undergone a significant transformation with the advent of Large Language Models (LLMs). These powerful models, often referred to as Generative AI (GenAI), have revolutionized how machines understand and generate human language, enabling unprecedented advancements in a wide array of applications, including hardware design verification. This paper presents an agentic AI-based approach to hardware design verification, which empowers AI agents, in collaboration with Humain-in-the-Loop (HITL) intervention, to engage in a more dynamic, iterative, and self-reflective process, ultimately performing end-to-end hardware design and verification. This methodology is evaluated on five open-source designs, achieving over 95% coverage with reduced verification time while demonstrating superior performance, adaptability, and configurability.

==> sections/results_new.tex <==
To evaluate the performance and benchmark the capabilities of our multi-agent framework, we applied it to generate and verify RTL designs for three security-relevant cores: CRC, ECC, and AES.
The design specifications for these benchmarks were derived from existing designs available on the OpenCores platform \cite{opencores}.
These designs were generated using the GPT-4o model from OpenAI \cite{openai2025chatgpt4o}, which comprises 1.8 trillion parameters, under three distinct temperature settings (0.2, 0.5, and 0.8). 
In the context of \acp{LLM}, the temperature parameter governs the randomness of the generated output. Lower temperature settings (e.g., 0.2) produce more deterministic and focused results, whereas higher temperatures (e.g., 0.8) introduce greater variability and creativity in the responses. 
For the RTL generation phase, performance was evaluated based on several criteria: the number of lint errors identified, the logical accuracy of the generated RTL (categorized as correct, correct but non-synthesizable, incorrect, or incomplete), and the \ac{HIL} effort required to render the RTL usable, measured in minutes. 
During the verification phase, key performance metrics included the number of generated properties, the formal coverage metric (\%), the number of \acp{CEX} identified, and the additional \ac{HIL} effort necessary to achieve near \SI{100}{\percent} coverage. 
The results, summarized in Table~\ref{tab:results_summary}, highlight the framework's efficiency and effectiveness in generating and verifying RTL designs across varying levels of complexity.



\begin{table}[ht]
	\centering
	\caption{Overview of the results}
	\begin{threeparttable}
		\adjustbox{width=\linewidth}{
			\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
				\hline
				\multirow{3}{*}{\textbf{Design}} & \multirow{3}{*}{\textbf{Temp}} & \multicolumn{4}{c|}{\textbf{RTL Generation}} & \multicolumn{6}{c|}{\textbf{Formal Property Generation}} \\ \cline{3-12} 
				&  & \multicolumn{2}{c|}{\textbf{\#Errors (linting)}} & \multicolumn{2}{c|}{\textbf{Logical Accuracy}} & \multicolumn{2}{c|}{\textbf{\#Properties}} & \multicolumn{2}{c|}{\textbf{Coverage (\%)}} & \multicolumn{2}{c|}{\textbf{\#CEXs}} \\ \cline{3-12}
				&  & \textbf{LLM} & \textbf{HIL} & \textbf{LLM} & \textbf{HIL} & \textbf{LLM} & \textbf{HIL} & \textbf{LLM} & \textbf{HIL} & \textbf{LLM} & \textbf{HIL} \\ \hline
				\multirow{3}{*}{CRC \cite{opencores}} & 0.2 & 0 & 0 & \faCheck & \faCheck & \multirow{3}{*}{16} & \multirow{3}{*}{11} & \multirow{3}{*}{73.08} & \multirow{3}{*}{100} & \multirow{3}{*}{8} & \multirow{3}{*}{0} \\ \cline{2-6}
				& 0.5 & 0 & 0 & \faExclamation & \faCheck &  &  &  &  &  &  \\ \cline{2-6}
				& 0.8 & 0 & 0 & \faTimes & \faCheck &  &  &  &  &  &  \\ \hline
				\multirow{3}{*}{ECC} & 0.2 & 5 & 0 & \faBan & \faCheck & \multirow{3}{*}{19} & \multirow{3}{*}{12} & \multirow{3}{*}{93.88} & \multirow{3}{*}{95.90*} & \multirow{3}{*}{8} & \multirow{3}{*}{0} \\ \cline{2-6}
				& 0.5 & 2 \faFlash & 0 & \faBan & \faCheck &  &  &  &  &  &  \\ \cline{2-6}
				& 0.8 & 2 \faFlash & 0 & \faBan & \faCheck &  &  &  &  &  &  \\ \hline
				\multirow{3}{*}{AES \cite{opencores}} & 0.2 & 0 & 0 & \faBan & \faCheck & \multirow{3}{*}{-} & \multirow{3}{*}{-} & \multirow{3}{*}{-} & \multirow{3}{*}{-} & \multirow{3}{*}{-} & \multirow{3}{*}{-} \\ \cline{2-6}
				& 0.5 & 0 & 0 & \faBan & \faCheck &  &  &  &  &  &  \\ \cline{2-6}
				& 0.8 & 1 \faFlash & 0 & \faBan & \faCheck &  &  &  &  &  &  \\ \hline
			\end{tabular}
		}
		\vspace{1mm} % Add space between the table and notes
		\begin{center}
			\scriptsize % Reduce font size for notes
			\faFlash: Fatal, \faCheck: Correct, \faExclamation: Non-synthesizable, \faTimes: Incorrect, \faBan: Incomplete. \\
			\vspace{1mm} % Add vertical spacing between symbols and effort descriptions
			\parbox{\columnwidth}{
				The HIL effort (in minutes) for RTL Generation and Formal Property Generation of CRC, ECC, and AES were 15/40, 30/20, and 45/90, respectively, across all Temp values. \\
				* Indicates unreachable dead code for 95.90\%.
			}
		\end{center}
	\end{threeparttable}
	\label{tab:results_summary}
\end{table}



\subsection{RTL Generation}

Our evaluation demonstrated that \acp{LLM} excel in code generation, particularly when multiple agents collaborate on the same task. 
For single-module designs, such as CRC, the generated RTL consistently exhibited no lint errors across all temperature settings. 
However, higher temperature settings introduced increased randomness, occasionally resulting in incorrect or incomplete RTL, as illustrated in Table~\ref{tab:results_summary}. These issues were efficiently addressed with minimal \ac{HIL} intervention, typically requiring less than 15 minutes to refine the RTL for usability. 
For ECC design, a temperature of 0.3 led to the generation of two design modules with placeholders in several functions, causing lint errors. By refining the specifications and adjusting agent configurations to provide additional context, these issues were effectively resolved. Subsequent \ac{HIL} efforts, amounting to under 30 minutes, successfully completed the missing functions, rendering the RTL usable. At higher temperature settings, ECC design exhibited more severe lint errors; however, these were promptly rectified through targeted \ac{HIL} actions. 
In the case of AES designs, multiple modules (ranging from three to five) were generated across varying temperature settings. At lower temperatures, the generated RTL contained placeholders that were subsequently completed. As the temperature increased, additional \ac{HIL} efforts were required to create predefined LUTs and complete missing functions, ensuring that the RTL met usability requirements. 
Overall, the framework demonstrated its robustness in reliably generating synthesizable RTL designs with manageable \ac{HIL} contributions. These results underscore the effectiveness of the multi-agent approach in addressing varying design complexities and mitigating temperature-induced variations.


\subsection{Formal Property Generation}

The lint-error-free RTL was subjected to formal verification using the Jasper tool, where the generated properties were validated, and coverage metrics were analyzed. 
For CRC, 16 properties were generated, achieving a proven rate with eight \acp{CEX} and an initial coverage of \SI{73.08}{\percent}. Through \ac{HIL} interventions involving 40 minutes of effort and the addition of new properties, coverage was elevated to \SI{100}{\percent}. 
Similarly, for ECC, 19 properties were generated, attaining a proven rate with eight \acp{CEX} and an initial coverage of \SI{93.88}{\percent}, as detailed in Table~\ref{tab:results_summary}. 
\ac{HIL} efforts totaling 20 minutes facilitated the incorporation of additional properties, thereby extending coverage to \SI{95.90}{\percent}. 
These interventions involved refining property specifications and addressing uncovered scenarios identified during the initial verification pass. 
\SI{100}{\percent} coverage was not achieved for ECC due to the presence of unreachable dead code. 
<Formal verification for AES is currently underway> 
The iterative process of property generation, validation, and refinement ensured comprehensive coverage and identified all critical issues within the RTL designs. 
This systematic approach highlights the framework’s capability to enhance formal verification outcomes through targeted human interventions, ensuring that the RTL designs meet stringent correctness and reliability standards derived directly from the design specifications.
\newline

The \ac{MAS} framework effectively leverages the strengths of \acp{LLM} and specialized agents to manage complex verification tasks. By decomposing the verification process into smaller, manageable segments, the framework mitigates common \acp{LLM} issues such as attention deficits, hallucinations, and iterative loops. 
\ac{HIL} interventions play a pivotal role in enhancing robustness by enabling the timely resolution of errors and completion of incomplete outputs generated by the \acp{LLM}. 
This collaboration between automated agents and human oversight ensures high accuracy and completeness in RTL generation and verification. 
Critic agents ensure the quality and correctness of generated properties through continuous feedback, enabling iterative improvements essential for refining \acp{SVA} and meeting formal verification metrics. 
Additionally, the framework’s ability to handle varying temperature settings demonstrates its adaptability to different levels of output randomness, enabling controlled experimentation and optimization of design generation processes. 
The minimal \ac{HIL} effort required to resolve issues across different designs underscores the efficiency of the multi-agent approach, significantly reducing the overall time and resources needed for RTL usability and verification. 
Overall, the framework’s systematic task division, agent specialization, and seamless human collaboration ensure comprehensive coverage, error-free RTL generation, and reliable verification outcomes. 
This makes it a robust and adaptable solution for hardware design and verification projects.

